Hedging Beyond the Mean: A Distributional Reinforcement Learning Perspective for Hedging Portfolios with Structured Products

Research in quantitative finance has demonstrated that reinforcement learning (RL) methods have delivered promising outcomes in the context of hedging financial portfolios. For example, hedging a portfolio of European options using RL achieves better $PnL$ distribution than the trading hedging strategies like Delta neutral and Delta-Gamma neutral [Cao et. al. 2020]. There is great attention given to the hedging of vanilla options, however, very little is mentioned on hedging a portfolio of structured products such as Autocallable notes. Hedging structured products is much more complex and the traditional RL approaches tend to fail in this context due to the underlying complexity of these products. These are more complicated due to presence of several barriers and coupon payments, and having a longer maturity date (from $7$ years to a decade), etc. In this direction, we propose a distributional RL based method to hedge a portfolio containing an Autocallable structured note. We will demonstrate our RL hedging strategy using American and Digital options as hedging instruments. Through several empirical analysis, we will show that distributional RL provides better $PnL$ distribution than traditional approaches and learns a better policy depicting lower value-at-risk ($VaR$) and conditional value-at-risk ($CVaR$), showcasing the potential for enhanced risk management.

==> related.tex <==
\section{Related Works}
\label{sec:related}

Recently, Reinforcement Learning (RL) based methods have been explored extensively in finance, for example, optimal trade execution~\cite{zhang2023generalizable_optimaltrade}, credit pricing~\cite{khraishi2022offline_creditpricing_icaif22}, market making~\cite{ganesh2019reinforcement_marketmaking}, learning exercise policies for American options~\cite{pmlr-v5-li09d_earlyexerciseRL}, optimal hedging~\cite{2q_Cao_2020,kolm_ritter,deeper_hedging_Gao_2023,murray2022deep_icaif22}, etc.  

Hedging a portfolio of exotic options is a fundamental research problem which requires sequential decision making to re-balance the portfolio at different intervals for hedging. This sequential decision making has attracted reinforcement learning based solutions which outperform traditional hedging strategies. For example, \cite{kolm_ritter} have used Deep Q-learning and Proximal Policy Optimization (PPO) algorithms in RL to learn a policy for option replications with market frictions. They learn a single policy which works with several strike prices. \cite{2021_giurca_delta} used RL for delta hedging under various parameters such as transaction cost, option maturity, and hedging frequency. They applied transfer learning to use the policy trained on simulated data for real data. \cite{2q_Cao_2020} and \cite{deeper_hedging_Gao_2023} used DDPG (Deep Deterministic Policy Gradient) RL algorithm to perform hedging under SABR and Heston volatility models respectively. 

\cite{2022_empirical_deep_hedging} trained an RL algorithm directly on real data for intraday options, over 6 years, on the $S\&P500$ index. \cite{jpmorgan_market_friction} hedged over-the-counter derivatives using RL algorithm under market frictions like trading cost and liquidity constraints. \cite{cva_hedge} used reinforcement learning for CVA hedging. The literature has given much attention on using RL based sequential decision making on several European~\cite{kolm_ritter,2q_Cao_2020,halperin2019qlbs}, American~\cite{pmlr-v5-li09d_earlyexerciseRL}, and Barrier options~\cite{chen2023hedging_barrier}. These methods have demonstrated that RL is an attractive alternative to traditional hedging strategies based on the performance and $PnL$ distribution. However, there is little attention on hedging very risky options such as Autocallable notes. Recently, \cite{autocall_hedge_mc} proposed a method for pricing Autocallable notes and employing a Delta neutral strategy for hedging. They emphasized that the hedging is very complicated due to presence of several barriers, noting the high cost of Delta hedging near these barriers. In contrast, our approach involves training a RL policy for hedging of a 7-year maturity Autocallable note portfolio. % Recently, \cite{autocall_hedge_mc} has proposed a method for the pricing of autocallable notes and hedging using Delta neutral strategy. As our observation, they emphasized that the hedging is very complicated due to presence of several barriers. They showed that Delta hedging is becomes very costly because the Delta value of the portfolio near the barrier is very high. Whereas, we learn a policy using RL to hedge such a portfolio of Autocallable note with a maturity of $7$ years. 
We show the performance of an RL agent under varying transaction cost and choosing different options as hedging instruments. We demonstrate that the RL agent provides better $PnL$ distribution than traditional hedging strategies. 

